Reassessing Java Code Readability Models with a Human-Centered Approach

To ensure that Large Language Models (LLMs) effectively support user productivity, they need to be adjusted. Existing Code Readability (CR) models can guide this alignment. However, there are concerns about their relevance in modern software engineering since they often miss the developers' notion of readability and rely on outdated code. This research assesses existing Java CR models for LLM adjustments, measuring the correlation between their and developers' evaluations of AI-generated Java code. Using the Repertory Grid Technique with 15 developers, we identified 12 key code aspects influencing CR that were consequently assessed by 390 programmers when labeling 120 AI-generated snippets. Our findings indicate that when AI generates concise and executable code, it is often considered readable by CR models and developers. However, a limited correlation between these evaluations underscores the importance of future research on learning objectives for adjusting LLMs and on the aspects influencing CR evaluations included in predictive models.

==> sections/3.2-aspects.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{@{}p{0.4\linewidth}p{0.4\linewidth}@{}}
\toprule
\textbf{Readable pole} & \textbf{Unreadable pole} \\
\midrule
\rowcolor{gray}
Code is concise & Code is too long \\
Code reads well from top to bottom & While reading, the eyes jump from top \newline to bottom and back up again \\
\rowcolor{gray}
\textasteriskcentered Code is not sufficiently explained and needs \newline additional info to understand what it does & Code is overexplained \\
The goal of the code is clear & The goal of the code is not clear \\
\rowcolor{gray}
Code uses basic, known code patterns & Code looks unfamiliar, non-standard \\
Functionality is separated logically & Code needs refactoring \\
\rowcolor{gray}
Code is flat and linear & Code is overly nested \\
There is one action per line of code & There are multiple actions on one line \\
\rowcolor{gray}
Code uses named constants & Code uses ``magic numbers'' \\
Naming clarifies code functionality & Naming is confusing \\
\rowcolor{gray}
Code conforms to style guides & Code is poorly formatted \\
There is balance in the color blocks & There are huge chunks of color blocks \newline that stand out in a distracting way \\
\bottomrule
\end{tabular}

\begin{tablenotes}
\centering
\footnotesize
    \item \textasteriskcentered This characteristic forms a continuum, being ``Readable'' in the middle and ``Unreadable'' at the extremes.    
\end{tablenotes}
\medskip
\caption{\CR Aspects.}
\label{tab:characteristics}
\end{table*}


==> sections/4.3-descr_experience.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lc@{}}
\hline
\textbf{Experience years} & \textbf{\# of participants} \\
\hline
Less than 1 year & 27 \\
1--2 years & 60 \\
3--4 years & 55 \\
5--6 years & 44 \\
7--8 years & 42 \\
9--10 years & 20 \\
More than 10 years & 142 \\
\hline
\end{tabular}
\smallskip
\caption{Programming Experience Distribution.}
\label{tab:prog_exp}

% \hspace{0.1\textwidth}
% \begin{minipage}{0.4\textwidth}
% \centering
% \begin{tabular}{@{}lc@{}}
% \hline
% \textbf{Experience level} & \textbf{\# of participants} \\
% \hline
% Beginner & 36 \\
% Intermediate & 162 \\
% Advanced & 192 \\
% \hline
% \end{tabular}
% \smallskip
% \caption{Java Experience Level Distribution.}
% \label{tab:exp_lvl}
% \end{minipage}
\vspace{-30pt}
\end{table}



==> sections/4.4-descr_prof.tex <==
\begin{table}[ht]
\centering

\begin{minipage}{0.4\textwidth}
\centering
\begin{tabular}{@{}lc@{}}
\hline
Language & \# of participants \\
\hline
Java & 390 \\
JavaScript & 207 \\
SQL (PL/SQL, T-SQL) & 177 \\
HTML / CSS & 163 \\
Python & 141 \\
TypeScript & 138 \\
Shell scripting languages & 116 \\
Kotlin & 111 \\
Go & 40 \\
C++ & 39 \\
\hline
\end{tabular}
\smallskip
\caption{Language Proficiency Distribution.}
\label{tab:lang_prof}
\end{minipage}
\hspace{0.1\textwidth}
\begin{minipage}{0.4\textwidth}
\centering
\begin{tabular}{@{}lc@{}}
\hline
Role & \# of participants \\
\hline
Developer & 362 \\
Architect & 62 \\
Team Lead & 61 \\
DevOps Engineer & 45 \\
Tester & 14 \\
\hline
\end{tabular}
\smallskip
\caption{Job Role Distribution.}
\label{tab:job_role}
\end{minipage}

\end{table}


==> sections/4.5-agreement.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lc@{}}
\hline
\textbf{Experience Level} & \textbf{Krippendorff's $\alpha$} \\
\hline
All Levels & 0.14 \\
Beginners & 0.04 \\
Intermediate & 0.10 \\
Advanced & 0.16 \\
\bottomrule
\end{tabular}
\smallskip
\caption{Krippendorff's $\alpha$ for Different Expert Groups.}
\label{tab:alpha}
\end{table}


==> sections/4.6-mcc.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lc@{}}
\toprule
\textbf{Model} & \textbf{MCC} \\
\midrule
Posnett's & -0.036 \\
Dorn's & -0.038 \\
Scalabrino's & 0.325 \\
Mi's & 0.033 \\
\bottomrule
\end{tabular}
\smallskip
\caption{Matthews correlation coefficient between \\model and human evaluations of \CR.}
\label{tab:mcc}
\end{table}

